RAG-DDR: Optimizing Retrieval-Augmented Generation Using Differentiable Data Rewards

Retrieval-Augmented Generation (RAG) has proven its effectiveness in mitigating hallucinations in Large Language Models (LLMs) by retrieving knowledge from external resources. To adapt LLMs for the RAG systems, current approaches use instruction tuning to optimize LLMs, improving their ability to utilize retrieved knowledge. This supervised fine-tuning (SFT) approach focuses on equipping LLMs to handle diverse RAG tasks using different instructions. However, it trains RAG modules to overfit training signals and overlooks the varying data preferences among agents within the RAG system. In this paper, we propose a Differentiable Data Rewards (DDR) method, which end-to-end trains RAG systems by aligning data preferences between different RAG modules. DDR works by collecting the rewards to optimize each agent in the RAG system with the rollout method, which prompts agents to sample some potential responses as perturbations, evaluates the impact of these perturbations on the whole RAG system, and subsequently optimizes the agent to produce outputs that improve the performance of the RAG system. Our experiments on various knowledge-intensive tasks demonstrate that DDR significantly outperforms the SFT method, particularly for LLMs with smaller-scale parameters that depend more on the retrieved knowledge. Additionally, DDR exhibits a stronger capability to align the data preference between RAG modules. The DDR method makes the generation module more effective in extracting key information from documents and mitigating conflicts between parametric memory and external knowledge. All codes are available at https://github.com/OpenMatch/RAG-DDR.

==> figure/evaluation_data.tex <==
\begin{figure}[t]        
    \centering
    \includegraphics[width = 1.0\textwidth] {image/evaluation_data.png}
    \caption{\label{fig:prompt_evaluation}Prompts Templates Used in Evaluation. }

\end{figure}

==> figure/intro.tex <==
\begin{figure}[t]        
    \centering
    \includegraphics[width = 1.0\textwidth] {image/intro1.png}
    \caption{\label{fig:intro}Illustrations of RAG Pipeline. }

\end{figure}

==> figure/knowledge_conflict.tex <==
\begin{figure}[t]
    \centering 
    \subfigure { 
    \label{fig:1} 
     \includegraphics[width=0.8\linewidth]{image/label.png}}
    \subfigure[The Answers Inclusion in Documents (NQ).] { 
    \label{fig:gold:nq} 
     \includegraphics[width=0.32\linewidth]{image/true_nq.png}}
     \subfigure[The Answers Exclusion in Documents (NQ).] { 
     \label{fig:bad:nq}
    \includegraphics[width=0.32\linewidth]{image/false_nq.png}}
    \subfigure[Internal and External Knowledge Conflicts (NQ).] { 
     \label{fig:an:nq}
     \includegraphics[width=0.32\linewidth]{image/noise_nq.png}}
    \subfigure[The Answers Inclusion in Documents (HotpotQA).] { 
     \label{fig:gold:hotpop}
    \includegraphics[width=0.32\linewidth]{image/true_hot.png}}
    \subfigure[The Answers Exclusion in Documents (HotpotQA).] { 
     \label{fig:bad:hotpop}
    \includegraphics[width=0.32\linewidth]{image/false_hot.png}}
     \subfigure[Internal and External Knowledge Conflicts  (HotpotQA).] { 
     \label{fig:an:hotpop}
    \includegraphics[width=0.32\linewidth]{image/noise_hot.png}}
    \caption{Effectiveness of Different Models in Utilizing Knowledge.}
    \vspace{-1em}
    \label{fig:conflict}
\end{figure}

==> figure/length.tex <==
\begin{figure}[t]        
    \centering
    \subfigure[The Output Length of RAG.] { 
    \label{fig:gen_lengthaa} 
     \includegraphics[width=0.32\linewidth]{image/length.png}}
     \subfigure[The Improvement Ratio of KR.] { 
     \label{fig:kr_improve}
    \includegraphics[width=0.32\linewidth]{image/rerank_difference.png}}
    \caption{Analyzing the Role of Modules in Data Reward Optimization. }

\end{figure}

==> table/ablation_order.tex <==
\begin{table}[t]
\caption{\label{tab:ablation_order}Ablation Study. We report MiniCPM-2.4B the top-5 retrieval-augmented results.}
\centering
\small
\begin{tabular}{l|ccc|c c|c|c}
\hline
\multirow{2}{*}{\textbf{Setting}} & \multicolumn{3}{c|}{\textbf{Open-domain QA}} & \multicolumn{2}{c|}{\textbf{Multi-Hop QA}} & \textbf{Slot Filling} & \textbf{Dialogue} \\ 
\cline{2-8}
& \textbf{NQ} & \textbf{TriviaQA} & \textbf{MARCO QA} & \textbf{HotpotQA}  & \textbf{Musique}  & \textbf{T-REx} & \textbf{WoW} \\ 
\hline
\multicolumn{8}{l}{\textit{Reward Model Selection}} \\
\hline
Generation & 46.1  & 81.9 & 28.2 &31.8  & &32.1 & 15.8  \\ 
DPO Generation  & 47.0  &82.7  &28.1  &32.5  & &32.6 & 15.7 \\ 
\hline
\multicolumn{8}{l}{\textit{Training Order}} \\
\hline
Generation First &  &  &  &  & & &  \\ 
Reranker First  &  &  &  &  & & &  \\ 
\hline
\end{tabular}

\end{table}

==> table/dpo_no_rag.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|ccc|c|c|c}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Open-domain QA}} & \multicolumn{1}{c|}{\textbf{Multi-Hop QA}} & \textbf{Slot Filling} & \textbf{Dialogue} \\ 
\cline{2-7}
& \textbf{NQ} & \textbf{TriviaQA} & \textbf{MARCO QA} & \textbf{HotpotQA}   & \textbf{T-REx} & \textbf{WoW} \\ 
\hline
\multicolumn{7}{l}{\textit{MiniCPM-2.4B}} \\
\hline
Vanilla LLM & 20.1  & 45.0  & 17.1  &  17.7 &  22.6 & 14.9  \\ 
RA-DIT & 18.4  & 43.1  & 20.5  &16.9   & 23.0  & 15.9  \\ 
DDR  & \textbf{21.6}  &\textbf{46.8}  &\textbf{21.4}  &\textbf{21.0}   &\textbf{23.4} & \textbf{16.8} \\ 
\hline
\multicolumn{7}{l}{\textit{Llama3-8B}} \\
\hline
Vanilla LLM & 35.4  & 78.4  &17.0  &27.7   &16.0 & 14.6 \\ 
RA-DIT & 33.5  & 74.8   &\textbf{22.2}  & 27.7  &\textbf{35.1}   &15.0   \\ 
DDR  & \textbf{37.3} & \textbf{79.2} &19.4 &\textbf{29.9}  & 25.7 &\textbf{15.8}  \\  
\hline
\end{tabular}
\caption{\label{tab:no_rag}Performance of Ours without Retrieval-Augmented Generation.}
\end{table}

==> table/overall_dspy.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textbf{HotPotQA }} & \multicolumn{2}{c|}{\textbf{MATH}} & \multicolumn{2}{c}{\textbf{HumanEval
}}\\ \cline{2-7}
& MiniCPM &Llama3 & MiniCPM &Llama3 & MiniCPM &Llama3 \\
\hline
LLMs &7.6/13.8 & 	&	&	&	&  \\ 
Agents &35.6/43.8  &  &  &  &  &  \\ 
DSPy  &35.0/43.9  &  &  &  & &   \\
Ours  &  &  &  &  & &   \\
\hline

\hline
\end{tabular}
\caption{\label{tab:overalldspy}1}
\end{table}
